L1 Optimal Control of Continuous-Time Stochastic Positive Systems

We present an L1-optimal control problem class with linear nonnegative costs subject to multiplicative It\^o diffusion processes with elementwise linear input constraints. Forward invariance of the positive orthant is established for the considered stochastic dynamics, and a simulation method consistent with this invariance property is proposed. Both finite-horizon and discounted infinite-horizon stochastic L1-optimal control problems are considered. These problems admit explicit solutions characterized by a vector-valued ordinary differential equation in the finite-horizon case and by an algebraic equation in the infinite-horizon case. Notably, the optimal value function and feedback policy coincide with those of the corresponding deterministic problem, demonstrating robustness to multiplicative stochastic uncertainty. A portfolio example illustrates our results.

==> mycommands.tex <==
\newcommand{\T}{^{\top}}
\newcommand{\inv}{^{-1}}
% \newcommand{\sign}{\operatorname{sign}}
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left]}
\renewcommand{\]}{\right]}
\renewcommand{\{}{\left{}
\renewcommand{\}}{\right}}
\newcommand{\sign}{\operatornamewithlimits{sign}}


